The TTC 2013 Flowgraphs Case

This case for the Transformation Tool Contest 2013 is about evaluating the scope and usability of transformation languages and tools for a set of four tasks requiring very different capabilities. One task deals with typical model-to-model transformation problem, there's a model-to-text problem, there are two in-place transformation problems, and finally there's a task dealing with validation of models resulting from the transformations. The tasks build upon each other, but the transformation case project also provides all intermediate models, thus making it possible to skip tasks that are not suited for a particular tool, or for parallelizing the work among members of participating teams.

==> eptcsdata.tex <==
\providecommand{\firstpage}{3}
\providecommand{\publicationstatus}{Pieter Van Gorp, Louis M. Rose, Christian Krause (Eds.):\\
Sixth Transformation Tool Contest (TTC 2013)\\
EPTCS 135, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.135.1}{10.4204/EPTCS.135.1}}
\pdfoutput=1

